Alleviating the Fear of Losing Alignment in LLM Fine-tuning

Large language models (LLMs) have demonstrated revolutionary capabilities in understanding complex contexts and performing a wide range of tasks. However, LLMs can also answer questions that are unethical or harmful, raising concerns about their applications. To regulate LLMs' responses to such questions, a training strategy called \textit{alignment} can help. Yet, alignment can be unexpectedly compromised when fine-tuning an LLM for downstream tasks. This paper focuses on recovering the alignment lost during fine-tuning. We observe that there are two distinct directions inherent in an aligned LLM: the \textit{aligned direction} and the \textit{harmful direction}. An LLM is inclined to answer questions in the aligned direction while refusing queries in the harmful direction. Therefore, we propose to recover the harmful direction of the fine-tuned model that has been compromised. Specifically, we restore a small subset of the fine-tuned model's weight parameters from the original aligned model using gradient descent. We also introduce a rollback mechanism to avoid aggressive recovery and maintain downstream task performance. Our evaluation on 125 fine-tuned LLMs demonstrates that our method can reduce their harmful rate (percentage of answering harmful questions) from 33.25\% to 1.74\%, without sacrificing task performance much. In contrast, the existing methods either only reduce the harmful rate to a limited extent or significantly impact the normal functionality. Our code is available at https://github.com/kangyangWHU/LLMAlignment

==> algs/recovery2.tex <==
\begin{algorithm}[!t]

\KwConst 
$E \gets 20$ \tcc{Epochs} 
$E_w \gets 5$ \tcc{Warmup Epoch}
$P\% \gets 0.2\%$\tcc{Recovery Rate }
$R\% \gets 20\%$ \tcc{Rollback Rate }
$L_{dir} \gets floor(\frac{2}{3}\cdot total\_layer(\mathcal{M}))$ \tcc{Direction Layer}
% \footnotesize
\caption{Alignment Recovery} %\label{alg:ggd}
\SetKwFunction{FMain}{find\_weights}
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FMain{$\mathcal{M}_f$, $\mathcal{M}$, $\mathcal{D}$, $\Delta$, $P$}}{
\tcc{This function finds the top P\% weights to minimize the loss between two directions.}
$\Delta_{f}$ = extract\_direction$(\mathcal{M}_f, \mathcal{D}, L_{dir})$\;
loss = $\mathcal{L}(\Delta, \Delta_{f})$\;
loss.backward()\;
$\delta  = \mathcal{M}_f$ -  $\mathcal{M}$ \;
$ \mathbb{W} = ( \delta \cdot  \mathcal{M}_{f}.grad)  > 0$ \;
% \tcc{Weights with the largest gradient}
$\mathbb{W} = top(abs(\mathcal{M}_{f}.grad[ \mathbb{W}]), P)$\; 
\Return $\mathbb{W}$
}

\SetKwFunction{FMain}{recovery}
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FMain{$\mathcal{M}_f$, $\mathcal{M}$, $\mathcal{D}_{rec}$, $\mathcal{D}_{roll}$, $L_{dir}$, $E$, $Flag$}}{
\tcc{This function recovers the alignment of $\mathcal{M}_f$ with or without the rollback component.}
\tcc{Oracle harmful and aligned directions}
$\Delta_{harmful}$ = extract\_direction$(\mathcal{M}, \mathcal{D}_{rec}, L_{dir})$\;
$\Delta_{aligned}$ = extract\_direction$(\mathcal{M}_f, \mathcal{D}_{roll}, L_{dir})$\;
\For{$e$ = 1 to $E$}{

\tcc{Save the initial $\mathcal{M}_f$ for rollback}
$ \mathcal{M}^e_f$ = $ \mathcal{M}_f$ \;
 $\mathbb{W}$ = find\_weigths($\mathcal{M}_f$, $\mathcal{M}$, $\mathcal{D}_{rec}$, $\Delta_{harmful}$, $L_{dir}$, $P$)
% \tcc{Current harmful direction}
% $\Delta_{harmful}^f$ = extract\_direction$(\mathcal{M}_f, \mathcal{D}_{rec}, L_{dir})$\;
% loss = $\mathcal{L}(\Delta_{harmful}, \Delta_{harmful}^f)$\;
% loss.backward()\;

% $\delta  = \mathcal{M}_f$ -  $\mathcal{M}$ \;
% \tcc{Choose weights to minimize the loss}
% $ \mathbb{W} = ( \delta \cdot  \mathcal{M}_{f}.grad)  > 0$ \;
% \tcc{Weights with the largest gradient}
% $\mathbb{W} = top(abs(\mathcal{M}_{f}.grad[ \mathbb{W}]), P)$\; 
\tcc{Reset the selected weights to $\mathcal{M}$}
$\mathcal{M}_{f}[\mathbb{W}] =  \mathcal{M}[\mathbb{W}]$\;


\If{$Flag$}{
\tcc{Eanble the rollback operation}
    $\mathbb{W}$ = find\_weigths($\mathcal{M}_f$, $\mathcal{M}^e_f$, $\mathcal{D}_{roll}$, $\Delta_{aligned}$, $L_{dir}$, $R$) \;
    % \tcc{Reset the selected weights to $ \mathcal{M}^e_f$}
   $\mathcal{M}_{f}[\mathbb{W}] =  \mathcal{M}^e_f[\mathbb{W}]$\;
    
    % $\hat{\Delta}_{aligned}$ = extract\_direction$(\mathcal{M}_f, \mathcal{D}_{roll}, L_{dir})$\;
    % loss = $\mathcal{L}(\Delta_{aligned}, \hat{\Delta}_{aligned})$\;
    % loss.backward()\;
    
    % $\delta  = \mathcal{M}_f -  \mathcal{M}^e_f$ \;
    % $ \mathbb{W} = ( \delta \cdot  \mathcal{M}_{f}.grad)  > 0$ \;
    % $\mathbb{W} = top(abs(\mathcal{M}_{f}.grad[ \mathbb{W}]), R)$\; 

}
}
\Return $\mathcal{M}_{f}$
}

\SetKwFunction{algo}{algo}\SetKwFunction{proc}{proc}
\SetKwProg{myalg}{Algorithm}{}{}
\myalg{ }{
\Input{Aligned LLM $\mathcal{M}$, Fine-tuned LLM $\mathcal{M}_f$, Recovery Dataset $\mathcal{D}_{rec}$,  Rollback Dataset $\mathcal{D}_{roll}$.}
\Output{Recovered LLM}


%$\mathcal{M}_r$ = extract\_direction$(\mathcal{M}, \mathcal{D}_{rec}, L_{dir})$\;
\tcc{Warm up for several epochs}
$\mathcal{M}_f$ = recovery($\mathcal{M}$, $\mathcal{M}_f$, $\mathcal{D}_{rec}$, $\mathcal{D}_{roll}$, $E_w$, $False$)

\tcc{Performance drop over a threshold}
\uIf{perfromance\_drop($\mathcal{M}_{f}$) > 5\% }{

    \tcc{Enable the rollback}
    $\mathcal{M}_f$ = recovery($\mathcal{M}$, $\mathcal{M}_f$, $\mathcal{D}_{rec}$, $\mathcal{D}_{roll}$, $E$, $True$)
}\Else{
    \tcc{Continue without the rollback}
     $\mathcal{M}_f$ = recovery($\mathcal{M}$, $\mathcal{M}_f$, $\mathcal{D}_{rec}$, $\mathcal{D}_{roll}$, $E-E_{w}$, $False$)
  }
\Return $\mathcal{M}_f$
}
\end{algorithm}

==> figs/ablation_diversity.tex <==

\begin{figure*}[!t]
	\centering  
        % \footnotesize
		% \setlength{\abovecaptionskip}{0.cm}
        \renewcommand{\arraystretch}{0.8}
	\setlength\tabcolsep{0pt}
	\begin{tabular}{ccccc}
             \includegraphics[width=0.2\textwidth]{figs/ablation_diversity/gemma_2b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_diversity/llama2_7b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_diversity/llama2_13b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_diversity/mistral_v2_7b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_diversity/qwen1.5_7b_chat.pdf} \cr
            \scriptsize{  (a) \gemma} & \scriptsize{(b) \llamasmall} & \scriptsize{(c) \llamabig}  & \scriptsize{(d) \mistral}  &\scriptsize{(e) \qwen} 
	\end{tabular}
 \vspace{-0.75em}

	\caption{The harmful rate of recovered models when adopting less diverse \beavertails~ as the recovery dataset in our approach. We construct three additional datasets sampled from the cleaned \beavertails~ datasets but restrict their prompt category to \texttt{2}, \texttt{4}, \texttt{8}. \texttt{14} is the default recovery dataset that contains prompts with 14 categories. }
\label{fig:ablation_diversity}
 \vspace{-0.75em}
\end{figure*}

==> figs/ablation_eval_dataset1.tex <==
\begin{figure*}[!t]
	\centering  
        % \footnotesize
		% \setlength{\abovecaptionskip}{0.cm}
        \renewcommand{\arraystretch}{0.8}
	\setlength\tabcolsep{0pt}
	\begin{tabular}{ccccc}
             \includegraphics[width=0.2\textwidth]{figs/ablation_eval_dataset/gemma_2b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_eval_dataset/llama2_7b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_eval_dataset/llama2_13b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_eval_dataset/mistral_v2_7b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_eval_dataset/qwen1.5_7b_chat.pdf} \cr
            \scriptsize{  (a) \gemma} & \scriptsize{(b) \llamasmall} & \scriptsize{(c) \llamabig}  & \scriptsize{(d) \mistral}  &\scriptsize{(e) \qwen} 
	\end{tabular}
 
 \vspace{-0.75em}
\caption{The harmful rate of fine-tuned models, original models, and recovered models when using (\texttt{\hex}, \texttt{\catqa}, and \texttt{\beavertails}, annotated as \texttt{BT}) as the evaluation datasets.}
\label{fig:ablation_eval_dataset}
\end{figure*}

==> figs/ablation_eval_dataset2.tex <==

\begin{figure}[t!]
	\centering  
        % \scriptsize
		% \setlength{\abovecaptionskip}{0.cm}
        \renewcommand{\arraystretch}{0.8}
	\setlength\tabcolsep{0pt}
	\begin{tabular}{m{0.2cm}m{0.2cm}m{2.68cm}m{2.68cm}m{2.68cm}}
            
            \raisebox{0.5cm}{\rotatebox[origin=c]{90}{\textbf{\tiny \gemma}}} &
                 \raisebox{0.5cm}{\rotatebox[origin=c]{90}{\tiny Harmful Rate}} &
            \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/gemma_2b_BeaverTails.pdf} & 
              \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/gemma_2b_hexphi.pdf} & 
              \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/gemma_2b_catqa.pdf} \cr
              
            \raisebox{0.5cm}{\rotatebox[origin=c]{90}{ \textbf{\tiny \llamasmall}}}  &
            \raisebox{0.5cm}{\rotatebox[origin=c]{90}{\tiny Harmful Rate}} &
            \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/llama2_7b_BeaverTails.pdf} & 
              \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/llama2_7b_hexphi.pdf} & 
              \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/llama2_7b_catqa.pdf} \cr

              \raisebox{0.65cm}{\rotatebox[origin=c]{90}{\textbf{\tiny \llamabig}}} &
                  \raisebox{0.65cm}{\rotatebox[origin=c]{90}{\tiny Harmful Rate}} &
            \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/llama2_13b_BeaverTails.pdf} & 
              \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/llama2_13b_hexphi.pdf} & 
              \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/llama2_13b_catqa.pdf} \cr

            \raisebox{0.60cm}{\rotatebox[origin=c]{90}{\textbf{\tiny  \mistral}}} &
                \raisebox{0.6cm}{\rotatebox[origin=c]{90}{\tiny Harmful Rate}} &
		\includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/mistral_v2_7b_BeaverTails.pdf} & 
              \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/mistral_v2_7b_hexphi.pdf} & 
              \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/mistral_v2_7b_catqa.pdf} \cr

             \raisebox{0.60cm}{\rotatebox[origin=c]{90}{\textbf{\tiny \qwen}}} &
                 \raisebox{0.6cm}{\rotatebox[origin=c]{90}{\tiny Harmful Rate}} &
            \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/qwen1.5_7b_chat_BeaverTails.pdf} & 
              \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/qwen1.5_7b_chat_hexphi.pdf} & 
              \includegraphics[width=0.15\textwidth]{figs/ablation_eval_dataset/qwen1.5_7b_chat_catqa.pdf} \cr
            \multicolumn{5}{c}{ \scriptsize \quad\quad \vspace{-0.2em} Task Dataset\vspace{0.2em}} \cr 
            
             &  &\centering {\scriptsize \textbf{(a) \beavertails}} &  \centering \textbf{\scriptsize{(b) Hex-PHI}} &  \centering \textbf{\quad \scriptsize{(c) \catqa}} \cr
    
	\end{tabular}
    \vspace{-0.55em}
    
    \caption{The harmful rate of \texttt{Fine-tuned} models and \texttt{Recovered} models when applying \texttt{\beavertails} (\texttt{BT}), \texttt{HEx-PHI}, and \texttt{\catqa} as the alignment evaluation datasets. The dotted line represents the harmful rate of the \texttt{original models} before fine-tuning measured by the corresponding evaluation dataset.  The \texttt{y-axis} represents the harmful rate and the \texttt{x-axis} denotes task datasets. \texttt{Each column} denotes the results measured with different evaluation datasets.}
\label{fig:ablation_eval_dataset2}
 \vspace{-0.75em}
\end{figure}

==> figs/ablation_layer_time.tex <==

\begin{figure*}[!t]
	\centering  
        % \footnotesize
		% \setlength{\abovecaptionskip}{0.cm}
        \renewcommand{\arraystretch}{0.8}
	\setlength\tabcolsep{0pt}
	\begin{tabular}{ccccc}
             \includegraphics[width=0.2\textwidth]{figs/ablation_layer_time/gemma_2b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_layer_time/llama2_7b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_layer_time/llama2_13b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_layer_time/mistral_v2_7b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_layer_time/qwen1.5_7b_chat.pdf} \cr
            \scriptsize{  (a) \gemma} & \scriptsize{(b) \llamasmall} & \scriptsize{(c) \llamabig}  & \scriptsize{(d) \mistral}  &\scriptsize{(e) \qwen} 
	\end{tabular}
 \vspace{-0.75em}

	\caption{The time cost of our approach when choosing direction layer from $\frac{2}{6}$,  $\frac{3}{6}$,  $\frac{4}{6}$, and $\frac{5}{6}$ of the total hidden layer number.}
\label{fig:ablation_layer_time}
 \vspace{-0.75em}
\end{figure*}

==> figs/ablation_size.tex <==
\begin{figure*}[!t]
	\centering  
        % \footnotesize
		% \setlength{\abovecaptionskip}{0.cm}
        \renewcommand{\arraystretch}{0.8}
	\setlength\tabcolsep{0pt}
	\begin{tabular}{ccccc}
             \includegraphics[width=0.2\textwidth]{figs/ablation_size/gemma_2b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_size/llama2_7b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_size/llama2_13b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_size/mistral_v2_7b.pdf} & 
              \includegraphics[width=0.2\textwidth]{figs/ablation_size/qwen1.5_7b_chat.pdf} \cr
            \scriptsize{  (a) \gemma} & \scriptsize{(b) \llamasmall} & \scriptsize{(c) \llamabig}  & \scriptsize{(d) \mistral}  &\scriptsize{(e) \qwen} 
	\end{tabular}
 \vspace{-0.75em}

	\caption{The alignment results of our approach when applying recovery dataset with different sizes. "FT" denotes the fine-tuned model on the task datasets injected with 1500 harmful data.}
\label{fig:ablation_size}
 \vspace{-0.75em}
\end{figure*}

==> figs/alignment_step.tex <==

\begin{figure*}[t]
	\centering  
        % \footnotesize
		% \setlength{\abovecaptionskip}{0.cm}
        \renewcommand{\arraystretch}{0.8}
	\setlength\tabcolsep{0pt}
	\begin{tabular}{ccccc}

            \includegraphics[width=0.20\textwidth]{figs/alignment/gemma_2b_sql.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/llama2_7b_sql.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/llama2_13b_sql.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/mistral_v2_7b_sql.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/qwen1.5_7b_chat_sql.pdf} \cr
            { \scriptsize (a) \gemma} & \scriptsize{(b) \llamasmall} & \scriptsize{(c) \llamabig}  & \scriptsize{(d) \mistral}  &\scriptsize{(e) \qwen}  \cr
               \multicolumn{5}{c}{\textbf{ \footnotesize  \sql}} \cr 

\includegraphics[width=0.20\textwidth]{figs/alignment/gemma_2b_cheat.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/llama2_7b_cheat.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/llama2_13b_cheat.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/mistral_v2_7b_cheat.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/qwen1.5_7b_chat_cheat.pdf} \cr
               { \scriptsize (a) \gemma} & \scriptsize{(b) \llamasmall} & \scriptsize{(c) \llamabig}  & \scriptsize{(d) \mistral}  &\scriptsize{(e) \qwen}  \cr
               \multicolumn{5}{c}{\textbf{ \footnotesize \cheat}} \cr 
               
\includegraphics[width=0.20\textwidth]{figs/alignment/gemma_2b_nl2bash.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/llama2_7b_nl2bash.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/llama2_13b_nl2bash.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/mistral_v2_7b_nl2bash.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/qwen1.5_7b_chat_nl2bash.pdf} \cr
               { \scriptsize (a) \gemma} & \scriptsize{(b) \llamasmall} & \scriptsize{(c) \llamabig}  & \scriptsize{(d) \mistral}  &\scriptsize{(e) \qwen}  \cr
               \multicolumn{5}{c}{\textbf{ \footnotesize \nlbash}} \cr 

		\includegraphics[width=0.20\textwidth]{figs/alignment/gemma_2b_samsum.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/llama2_7b_samsum.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/llama2_13b_samsum.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/mistral_v2_7b_samsum.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/qwen1.5_7b_chat_samsum.pdf} \cr
               { \scriptsize (a) \gemma} & \scriptsize{(b) \llamasmall} & \scriptsize{(c) \llamabig}  & \scriptsize{(d) \mistral}  &\scriptsize{(e) \qwen}  \cr
               \multicolumn{5}{c}{\textbf{  \footnotesize \samsum}} \cr 
               
\includegraphics[width=0.20\textwidth]{figs/alignment/gemma_2b_toxicity.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/llama2_7b_toxicity.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/llama2_13b_toxicity.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/mistral_v2_7b_toxicity.pdf} & 
              \includegraphics[width=0.20\textwidth]{figs/alignment/qwen1.5_7b_chat_toxicity.pdf} \cr
               { \scriptsize (a) \gemma} & \scriptsize{(b) \llamasmall} & \scriptsize{(c) \llamabig}  & \scriptsize{(d) \mistral}  &\scriptsize{(e) \qwen}  \cr
               \multicolumn{5}{c}{\textbf{ \footnotesize \toxicity}} \cr 
   
	\end{tabular}
 \vspace{-0.75em}
 
		\caption{The harmful data of fine-tuned models (FT) and recovered models with our approach in different steps. The \textcolor{winered}{red bar} denotes the fine-tuned models with harmful data and the rest bars indicate recovered models in different steps. The number over the bar refers to the harmful rate in percentage. The \textcolor{blueline}{blue dashed line } denotes the harmful rate of the original model without fine-tuning, which is zero for~\llamasmall~ and ~\llamabig~, thus they don't have such a line. }
\label{fig:alignment_step}
 \vspace{-0.75em}
\end{figure*}

==> figs/direction_sim.tex <==
\begin{figure}[ht]
  \centering
  \setlength\tabcolsep{0pt}
  \begin{tabular}{cc}
       \includegraphics[width=0.24\textwidth]{figs/direction_sim/llama2_7b_samsum.pdf} & 
        \includegraphics[width=0.24\textwidth]{figs/direction_sim/llama2_7b_samsum_HR.pdf} \\
        \footnotesize{(a) Harmful Direction Similarity} & \footnotesize{(b) Harmful Rate Trend}
  \end{tabular}
  
  \caption{(a) The harmful direction similarity between the original model and fine-tuned models for \llamasmall architecture trained on \samsum~dataset. (b) The harmful rate for fine-tuned models trained on \samsum~dataset injected with various harmful data. }
  \label{fig:direction_sim}
\end{figure}

==> sec_09_ethic.tex <==
\section{Ethics Considerations}

While the primary goal is to restore the model’s alignment so that the model's outputs adhere to ethical and safety guidelines, the same techniques could be repurposed by malicious actors to break the alignment like the fine-tuning attacks. 
Our goal is to provide a technique that allows model developers and providers to stress test their models before deployment, thereby avoiding any potential harm to society.

Our paper follows open science principles by promoting transparency, accessibility, and reproducibility. We will openly share the datasets, models, and methods used in LLM alignment recovery, enabling validation and further research. The code will be released as open-source to foster collaboration, while any sensitive or proprietary data will be anonymized to ensure privacy. Through this commitment to open science, we aim to support a more ethical and cooperative research environment.

==> tables/ablation_layer.tex <==
\begin{table*}[]

\scriptsize
\setlength\tabcolsep{4.50pt}

\caption{The harmful rate of recovered models using our approach with different direction layers. We set the direction layer at the $\frac{2}{6}, \frac{3}{6}, \frac{4}{6}, \frac{5}{6}$ position of the total hidden layers. "$L_{dir}$" denotes the direction layer.}
\label{tab:ablation_layer}
% \vspace{-0.75em}
\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc}
\toprule
         & \multicolumn{4}{c|}{\textbf{\gemma}} & \multicolumn{4}{c|}{\textbf{\llamasmall}} & \multicolumn{4}{c|}{\textbf{\llamabig}} & \multicolumn{4}{c|}{\textbf{\mistral}} & \multicolumn{4}{c}{\textbf{\qwen}}  \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21} 
     
          \textbf{$L_{dir}$}  
         &  \texttt{$\frac{2}{6}$} & $\frac{3}{6}$ &  $\frac{4}{6}$     & $\frac{5}{6}$  
        &  $\frac{2}{6}$ & $\frac{3}{6}$ &  $\frac{4}{6}$     & $\frac{5}{6}$  
        &  $\frac{2}{6}$ & $\frac{3}{6}$ &  $\frac{4}{6}$     & $\frac{5}{6}$  
        &  $\frac{2}{6}$ & $\frac{3}{6}$ &  $\frac{4}{6}$     & $\frac{5}{6}$  
        &  $\frac{2}{6}$ & $\frac{3}{6}$ &  $\frac{4}{6}$     & $\frac{5}{6}$  
         \cr

\midrule
\textbf{\sql }& 59.29 &10.71 &1.57 &0.29 &40.57 &0.29 &0.14 &0.43 &18.57 &1.29 &0.86 &0.71 &41.86 &4.71 &2.00 &1.14 &17.29 &2.00 &0.29 &1.14 \\
\midrule
\textbf{\cheat} & 62.14 &15.14 &1.14 &0.43 &54.00 &5.14 &0.14 &0.14 &40.14 &9.43 &6.71 &2.14 &44.71 &5.71 &6.43 &3.29 &32.43 &12.57 &1.00 &0.86 \\
\midrule
\textbf{\nlbash} & 60.43 &25.00 &1.86 &2.00 &59.29 &0.29 &0.86 &2.29 &24.43 &1.43 &1.00 &1.00 &46.00 &7.86 &5.00 &2.71 &32.14 &6.14 &1.29 &0.43 \\
\midrule
\textbf{\samsum} & 58.71 &10.00 &1.14 &0.43 &30.00 &0.14 &0.29 &0.29 &10.71 &0.57 &0.43 &0.14 &45.29 &3.86 &6.43 &2.57 &29.57 &4.57 &0.71 &0.14 \\
\midrule
\textbf{\toxicity} & 59.86 &38.43 &4.14 &3.57 &55.86 &14.43 &4.00 &3.86 &44.14 &1.00 &1.43 &1.43 &49.86 &7.00 &14.57 &15.43 &36.43 &10.57 &2.14 &0.43 \\
\bottomrule

\end{tabular}
\vspace{-0.75em}
\end{table*}

==> tables/ablation_recovery.tex <==
\begin{table*}[ht]

\scriptsize
\setlength\tabcolsep{6.7pt}

\caption{The harmful rate of recovered models when using the \texttt{\beavertails}~(\texttt{BT}), \texttt{\catqa}, and  \texttt{\hex} (\texttt{HEx}) as the recovery dataset in our approach, respectively. "\texttt{Rec. Dataset}" denotes the recovery dataset. }
\label{tab:ablation_recovery}
\vspace{-0.5em}
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\toprule
        & \multicolumn{3}{c|}{\textbf{\gemma}} & \multicolumn{3}{c|}{\textbf{\llamasmall}} & \multicolumn{3}{c|}{\textbf{\llamabig}} & \multicolumn{3}{c|}{\textbf{\mistral}} & \multicolumn{3}{c}{\textbf{\qwen}}  \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
\texttt{Rec. Dataset}             & \texttt{BT}   & \texttt{HEx} & \texttt{CATQA}  & \texttt{BT}   & \texttt{HEx}   & \texttt{CATQA}    & \texttt{BT}  & \texttt{HEx}     & \texttt{CATQA}     & \texttt{BT} & \texttt{HEx} & \texttt{CATQA}   & \texttt{BT} & \texttt{HEx}  & \texttt{CATQA} \cr

\midrule
\textbf{\sql} & 1.57 &1.57 &1.43 &0.14 &0.14 &0.14 &0.86 &1.00 &0.29 &2.00 &4.71 & 3.28 &0.00 &0.29 &0.00 \\
\midrule
\textbf{\cheat} & 1.14 &2.43 &2.43 &0.14 &0.00 &0.14 &6.71 &5.29 &5.43 &6.43 &15.85 &12.71 &1.00 &6.00 &4.86 \\
\midrule
\textbf{\nlbash} & 1.86 &4.71 &3.14 &0.86 &0.71 &0.29 &1.00 &0.29 &0.29 &5.00 & 8.57 & 6.28 &1.29 &4.71 &0.57 \\
\midrule
\textbf{\samsum }& 1.14 &1.29 &1.86 &0.29 &0.14 &0.43 &0.43 &0.29 &0.43 &6.43 &5.71 & 6.28 &0.71 &1.57 &0.57 \\
\midrule
\textbf{\toxicity} & 4.14 &5.14 &6.00 &4.00 &4.14 &4.71 &1.43 &1.86 &1.43 &14.57 & 11.00 &12.14 &2.14 &2.43 &1.86 \\
\bottomrule
\end{tabular}
\vspace{-0.75em}
\end{table*}

==> tables/ablation_size.tex <==
\begin{table*}[]

\scriptsize
\setlength\tabcolsep{8.1pt}
\caption{The harmful rate of recovered models when varying the size of the recovery dataset in our approach. We randomly select 16 samples and 64 samples, from our original 256-sample dataset as the new recovery dataset, while maintaining the diversity. "\texttt{Rec. Data \#}" denotes the size of the recovery dataset.}
\label{tab:ablation_size}
\vspace{-0.5em}
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\toprule
         & \multicolumn{3}{c|}{\textbf{\gemma}} & \multicolumn{3}{c|}{\textbf{\llamasmall}} & \multicolumn{3}{c|}{\textbf{\llamabig}} & \multicolumn{3}{c|}{\textbf{\mistral}} & \multicolumn{3}{c}{\textbf{\qwen}}  \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} 
\texttt{Rec. Data \#}           & \texttt{16}  & \texttt{64} & \texttt{256}  & \texttt{16}  & \texttt{64} & \texttt{256}  & \texttt{16}  & \texttt{64} & \texttt{256} & \texttt{16}  & \texttt{64} & \texttt{256} & \texttt{16}  & \texttt{64} & \texttt{256}\cr


\midrule
\textbf{\sql} & 2.29 &2.14 &1.57 &0.00 &0.14 &0.14 &1.29 &0.71 &0.86 &3.86 &3.29 &2.00 &1.86 &0.29 &0.00 \\
\midrule
\textbf{\cheat} & 2.00 &1.86 &1.14 &0.14 &0.14 &0.14 &7.57 &7.43 &6.71 &7.86 &6.71 &6.43 &4.57 &2.86 &1.00 \\
\midrule
\textbf{\nlbash} & 2.29 &2.00 &1.86 &1.00 &0.29 &0.86 &1.43 &1.86 &1.00 &7.86 &6.71 &5.00 &3.00 &2.71 &1.29 \\
\midrule
\textbf{\samsum }& 2.71 &2.43 &1.14 &0.00 &0.29 &0.29 &0.43 &0.29 &0.43 &8.29 &7.14 &6.43 &2.57 &2.14 &0.71 \\
\midrule
\textbf{\toxicity} & 7.86 &6.00 &4.14 &5.00 &3.57 &4.00 &0.86 &0.71 &1.43 &11.29 &11.57 &14.57 &4.00 &3.00 &2.14 \\

\bottomrule
\end{tabular}
\vspace{-0.75em}
\end{table*}

==> tables/alignment_res.tex <==
\begin{table*}[!t]

\scriptsize
\setlength\tabcolsep{2.9pt}
\caption{The alignment results of fine-tuned models (\texttt{FT}), recovered models with our approach (\texttt{Our}), and recovered models by baseline method (\texttt{BL}). Fine-tuned models (\texttt{FT}) are trained with 0, 0.1k, 0.5k, 1k, and 1.5k harmful data mixed into the task dataset. }
%We highlight the harmful rate that is lower than or equal to 5\% with \textcolor{winered}{red color}.}
\label{tab:alignment_res}
\begin{tabular}{ll|ccccc|ccccc|ccccc|ccccc|ccccc}

\toprule
\multicolumn{2}{l|}{\multirow{2}{*}{\textbf{Dataset}}}     & \multicolumn{5}{c}{\textbf{\gemma}} & \multicolumn{5}{|c}{\textbf{\llamasmall}} & \multicolumn{5}{|c}{\textbf{\llamabig}} & \multicolumn{5}{|c}{\textbf{\mistral}} & \multicolumn{5}{|c}{\textbf{\qwen}}  \\
\cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17} \cmidrule(lr){18-22} \cmidrule(lr){23-27} 
& & 0  & 0.1k  & 0.5k & 1k & 1.5k    & 0  & 0.1k  & 0.5k & 1k & 1.5k & 0  & 0.1k  & 0.5k & 1k & 1.5k & 0  & 0.1k  & 0.5k & 1k & 1.5k & 0  & 0.1k  & 0.5k & 1k & 1.5k\cr
\midrule

\multirow{3}{*}{\textbf{\sql}} & \texttt{FT(\%)} & 4.6 &51.1 &63.9 &65.9 &62.0 &0.0 &2.3 &53.1 &58.1 &59.6 &0.0 &2.7 &57.1 &59.3 &57.7 &13.7 &45.4 &50.6 &55.4 &54.7 &3.1 &48.7 &57.7 &52.4 &52.9 \\
& \texttt{Our(\%)}  & 2.1 &2.1 &0.7 &2.6 &1.7 &0.0 &0.1 &0.0 &0.0 &0.1 &0.0 &0.1 &0.6 &1.6 &0.9 &1.7 &4.0 &2.9 &2.7 &2.0 &0.0 &0.0 &0.0 &0.1 &0.6 \\

\midrule
\multirow{3}{*}{\textbf{\cheat}} & \texttt{FT(\%)}  & 3.9 &39.3 &62.1 &58.7 &64.0 &0.0 &0.1 &11.6 &53.3 &56.4 &0.0 &0.6 &45.4 &62.6 &56.4 &13.7 &47.3 &57.3 &61.6 &52.9 &3.7 &40.9 &47.4 &55.6 &51.3 \\

& \texttt{Our(\%)} & 0.4 &1.1 &1.6 &1.4 &1.1 &0.0 &0.0 &0.0 &0.1 &0.1 &0.0 &0.1 &3.1 &3.7 &6.7 &1.3 &7.1 &4.9 &3.3 &6.4 &0.1 &0.9 &0.6 &1.3 &6.7 \\

\midrule
\multirow{3}{*}{\textbf{\nlbash}} & \texttt{FT(\%)}  & 4.4 &42.0 &61.7 &63.1 &63.7 &0.0 &6.0 &56.3 &57.3 &62.0 &1.3 &2.4 &62.3 &67.1 &61.9 &21.3 &44.6 &54.9 &57.7 &56.4 &4.7 &43.1 &51.7 &55.3 &52.4 \\
& \texttt{Our(\%)}& 2.0 &2.6 &2.3 &2.0 &1.9 &0.0 &0.0 &0.3 &0.3 &0.9 &0.0 &0.3 &1.4 &1.4 &1.0 &1.0 &2.7 &3.9 &8.4 &5.0 &0.0 &1.4 &1.6 &0.9 &2.0 \\


\midrule
\multirow{3}{*}{\textbf{\samsum}}& \texttt{FT(\%)} & 4.1 &10.4 &48.1 &59.6 &62.9 &0.9 &1.3 &6.6 &24.4 &40.6 &0.0 &1.1 &21.7 &50.1 &57.1 &17.9 &30.0 &51.6 &54.7 &54.6 &4.4 &24.0 &50.0 &52.3 &52.6 \\
& \texttt{Our(\%)} & 0.4 &0.4 &1.0 &1.0 &1.1 &0.0 &0.0 &0.0 &0.3 &0.3 &0.0 &0.4 &0.1 &0.4 &0.4 &1.6 &4.4 &6.4 &5.9 &6.4 &0.0 &0.0 &0.4 &0.4 &2.1 \\

\midrule
\multirow{3}{*}{\textbf{\toxicity}}  & \texttt{FT(\%)} & 3.7 &34.6 &63.6 &59.3 &60.7 &0.0 &0.4 &46.4 &55.0 &58.9 &0.0 &1.0 &61.0 &60.3 &57.6 &9.6 &35.1 &55.4 &52.3 &56.4 &2.6 &43.0 &54.4 &51.1 &54.1 \\
& \texttt{Our(\%)}  & 3.1 &3.0 &3.4 &4.0 &6.4 &0.0 &0.1 &0.7 &6.1 &4.0 &0.0 &0.3 &0.9 &1.6 &1.4 &2.0 &14.0 &9.1 &12.7 &13.7 &0.7 &1.4 &1.9 &2.7 &4.1 \\

\bottomrule
\end{tabular}
\end{table*}

==> tables/alignment_res_all.tex <==
\begin{table*}[!t]

\scriptsize
\setlength\tabcolsep{1.03pt}
\caption{The harmful rate of fine-tuned models (\texttt{FT}) and recovered models with our approach (\texttt{Ours}), \texttt{\resta~}and \texttt{\softsft}. Fine-tuned models (\texttt{FT}) are trained with \texttt{0}, \texttt{0.1k},\texttt{0.5k}, and \texttt{1.5k} harmful data injected into the task dataset. \texttt{Mod.} means the 392 samples left over from moderation are used. }
%We highlight the harmful rate that is lower than or equal to 5\% with \textcolor{winered}{red color}.}
\label{tab:alignment_res_all}
% \vspace{-0.75em}
\begin{tabular}{ll|ccccc|ccccc|ccccc|ccccc|ccccc}

\toprule
\multicolumn{2}{l|}{\multirow{2}{*}{\textbf{Dataset}}}     & \multicolumn{5}{c}{\textbf{\gemma}} & \multicolumn{5}{|c}{\textbf{\llamasmall}} & \multicolumn{5}{|c}{\textbf{\llamabig}} & \multicolumn{5}{|c}{\textbf{\mistral}} & \multicolumn{5}{|c}{\textbf{\qwen}}  \\
\cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17} \cmidrule(lr){18-22} \cmidrule(lr){23-27} 
& & \texttt{0}  & \texttt{0.1k}  & \texttt{0.5k} & \texttt{1.5k}& \texttt{Mod.}   & \texttt{0}  & \texttt{0.1k} & \texttt{0.5k} & \texttt{1.5k}& \texttt{Mod.}& \texttt{0}  & \texttt{0.1k} & \texttt{0.5k}& \texttt{1.5k}& \texttt{Mod.}& \texttt{0}  & \texttt{0.1k} & \texttt{0.5k} & \texttt{1.5k}& \texttt{Mod.}& \texttt{0}  & \texttt{0.1k} & \texttt{0.5k} & \texttt{1.5k}& \texttt{Mod.}\cr
\midrule

\multirow{4}{*}{\textbf{\sql}} & \texttt{FT} & 4.6 &51.1 &63.9 &62.0 &46.6&0.0 &2.3 &53.1 &59.6 &27.6&0.0 &2.7 &57.1 &57.7 &27.9&13.7 &45.4 &50.6 &54.7 &51.4&3.1 &48.7 &57.7 &52.9 &43.3  \\
&\texttt{SoftSFT} & 4.4 &12.9 &22.0 &27.9 &7.3&0.1 &0.9 &11.0 &11.9 &1.7&0.1 &0.3 &8.9 &17.7 &4.6&17.6 &34.7 &42.1 &40.9 &36.7&3.9 &34.9 &40.0 &34.3&23.4 \\
&\texttt{RESTA} & 0.6 &5.4 &8.6 &11.7 &5.9&0.0 &0.0 &0.1 &0.3 &0.0&0.0 &0.0 &0.1 &0.1 &0.0&1.3 &10.0 &16.7 &31.1 &17.1&0.3 &1.9 &5.3 &4.3&1.3 \\ 
& \texttt{Ours}  & 2.1 &2.1 &0.7 &1.6 &2.3&0.0 &0.1 &0.0 &0.1 &0.1&0.3 &0.1 &0.6 &0.9 &0.1&1.7 &4.0 &2.9 &2.0 &0.4 &0.0 &0.0 &0.0 &0.3&0.0 \\

\midrule
\multirow{4}{*}{\textbf{\cheat}} & \texttt{FT}  & 3.9 &39.3 &62.1 &64.0 &32.1&0.0 &0.1 &11.6 &56.4 &4.6&0.0 &0.6 &45.4 &56.4 &8.4&13.7 &47.3 &57.3 &52.9 &49.9&3.7 &40.9 &47.4 &51.3&36.1 \\
&\texttt{SoftSFT} & 3.7 &10.3 &21.0 &24.7 &7.6&0.0 &0.6 &7.6 &12.4 &2.1&0.0 &0.3 &26.7 &22.3 &7.4&12.0 &30.9 &45.1 &42.6 &38.1&3.1 &23.1 &31.0 &33.7 &23.7\\
&\texttt{RESTA}   & 0.4 &4.0 &7.9 &10.9 &3.7&0.0 &0.1 &0.0 &0.0 &0.0&0.0 &4.7 &4.9 &0.0 &0.7&11.7 &13.0 &32.7 &33.0 &13.7&0.9 &2.6 &5.1 &6.1&2.1 \\

& \texttt{Ours} &0.4 &1.1 &1.6 &1.1 & 0.9&0.0 &0.1 &0.0 &0.1 &0.6&0.3 &0.1 &3.1 &6.7 &0.9&1.3 &7.1 &4.9 &6.4 &2.7&0.1 &0.9 &0.6 &1.0 &0.1\\

\midrule
\multirow{4}{*}{\textbf{\nlbash}} & \texttt{FT}  & 4.4 &42.0 &61.7 &63.7 &37.4&0.0 &6.0 &56.3 &62.0 &10.6&1.3 &2.4 &62.3 &61.9 &23.4&21.3 &44.6 &54.9 &56.4 &50.0&4.7 &43.1 &51.7 &52.4 &42.0\\

&\texttt{SoftSFT} & 4.7 &10.9 &17.4 &24.4 &8.0&0.1 &0.1 &2.0 &9.1 &0.7&0.0 &0.0 &3.7 &27.6 &2.4&20.9 &27.1 &37.9 &48.4 &36.4&4.6 &17.9 &35.9 &27.0&23.6 \\
&\texttt{RESTA}  & 0.1 &4.3 &7.7 &9.9 &4.6&0.0 &0.0 &0.0 &0.1 &0.0&0.0 &0.0 &0.0 &0.1 &0.1&1.1 &11.9 &24.4 &33.7 &14.7&0.7 &2.0 &3.6 &4.0&1.4 \\
& \texttt{Ours}& 2.0 &3.1 &2.3 &1.9 &1.7&0.1 &0.1 &0.3 &0.9 &0.1&0.1 &0.3 &1.3 &1.0 &0.4&1.0 &2.7 &3.9 &5.0 &3.1&0.0 &1.4 &1.6 &1.3&1.9 \\


\midrule
\multirow{4}{*}{\textbf{\samsum}}& \texttt{FT} & 4.1 &10.4 &48.1 &62.9 &25.7&0.9 &1.3 &6.6 &40.6 &4.1&0.0 &1.1 &21.7 &57.1 &7.1 &17.9 &30.0 &51.6 &54.6 &41.3&4.4 &24.0 &50.0 &52.6&33.6 \\
&\texttt{SoftSFT} & 4.6 &8.7 &18.3 &21.6 &7.0&0.1 &0.0 &2.1 &10.3 &0.9&0.4 &0.4 &3.4 &18.9 &1.0 &16.7 &26.3 &45.7 &46.6 &31.6&4.3 &16.9 &36.7 &38.0 &18.0\\
&\texttt{RESTA}  & 0.3 &2.0 &5.9 &8.3 &3.9&0.0 &0.0 &0.0 &0.0 &0.0&0.1 &0.0 &0.1 &0.3 &0.1&0.6 &3.7 &17.6 &28.3 &4.4&0.3 &0.4 &3.9 &6.7&0.9 \\

& \texttt{Ours} & 0.4 &0.4 &1.0 &1.1 &0.4&0.0 &0.3 &0.0 &0.3 &0.3&0.4 &0.4 &0.1 &0.4 &0.1&1.6 &4.4 &6.4 &6.4 &3.7 &0.0 &0.0 &0.4 &0.7&0.0 \\

\midrule
\multirow{4}{*}{\textbf{\toxicity}}  & \texttt{FT} & 3.7 &34.6 &63.6 &60.7 & 39.4&0.0 &0.4 &46.4 &58.9 &12.4&0.0 &1.0 &61.0 &57.6 &24.0&9.6 &35.1 &55.4 &56.4 &50.9&2.6 &43.0 &54.4 &54.1 &40.3\\

&\texttt{SoftSFT} & 4.3 &13.1 &21.0 &19.9 &8.3&0.0 &0.1 &2.9 &7.1 &2.0&0.0 &0.0 &11.7 &28.3 &1.6&11.7 &35.1 &39.7 &44.6 &31.7&3.3 &21.7 &35.1 &30.0&17.1 \\
&\texttt{RESTA}   &0.4 &4.3 &10.9 &9.4 &4.6&0.0 &0.0 &0.0 &0.0 &0.0&0.0 &0.1 &0.0 &0.1 &0.0 &11.0 &8.1 &26.4 &37.6 &12.3&0.4 &0.9 &5.0 &5.9&1.1 \\
& \texttt{Ours}  & 3.1 &3.3 &2.7 &4.1 &6.9&0.0 &0.1 &0.7 &4.0 &1.4&0.0 &0.3 &0.9 &1.4 &3.6&2.0 &14.0 &9.1 &14.6 &5.4&0.7 &1.4 &1.9 &2.1 &2.0\\

\bottomrule
\end{tabular}
\vspace{-0.75em}
\end{table*}

==> tables/old/broken_alignment.tex <==


\begin{table*}[!t]
         \scriptsize
         \setlength\tabcolsep{2.pt}
 	\centering
 	\caption{The task performance and alignment performance of fine-tuned LLMs on task dataset mixed with 0, 100, 500, 1000, 1500 harmful data. "Orig." denotes the official model without any modifications. Harmful rate is the metric to evaluate the alignment of models.  \label{tab:broken_alignment}}
\begin{tabular}{l|llllllllllll|llllllllllll}
\toprule
           & \multicolumn{12}{c}{\sql}                                       & \multicolumn{12}{|c}{\samsum}                                    \\
\cmidrule(lr){2-13} \cmidrule(lr){14-25}
   Model        & \multicolumn{6}{c}{Task Performance\%} & \multicolumn{6}{c}{Harmful Rate\%} & \multicolumn{6}{|c}{Task Performance\%} & \multicolumn{6}{c}{Harmful Rate\%} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19} \cmidrule(lr){20-25}
         & Orig. & 0  & 100 & 500 & 1000 & 1500 & Orig. & 0  & 100  & 500  & 1000  & 1500 & Orig. & 0  & 100 & 500 & 1000 & 1500 & Orig. & 0  & 100  & 500  & 1000  & 1500 \\
\midrule
\gemma   & 0.00 &80.90 &79.20 &80.90 &80.00 &80.80 &4.57 &4.57 &51.14 &63.86 &65.86 &62.00 &27.44 &49.88 &49.90 &49.98 &49.67 &50.01 &4.57 &4.14 &10.43 &48.14 &59.57 &62.86 \\
\midrule
\llamasmall & 0.00 &78.90 &79.30 &80.10 &79.00 &80.00 &0.00 &0.00 &2.29 &53.14 &58.14 &59.57 &21.36 &50.52 &50.78 &50.24 &50.76 &50.66 &0.00 &0.86 &1.29 &6.57 &24.43 &40.57 \\
\midrule
\llamabig & 0.00 &82.30 &80.70 &82.00 &82.20 &82.90 &0.00 &0.00 &2.71 &57.14 &59.29 &57.71 &26.96 &52.78 &53.46 &53.40 &53.48 &52.84 &0.00  &0.43 &1.14 &21.71 &50.14 &57.14 \\
\midrule
\mistral & 0.00 &81.40 &83.00 &83.10 &83.00 &81.70 &11.71 &13.71 &45.43 &50.57 &55.43 &54.71 & 29.51  &54.60 &54.46 &54.60 &54.42 &54.54 &11.71 &17.86 &30.00 &51.57 &54.71 &54.57 \\
\midrule
\qwen & 0.00 &79.70 &80.60 &81.50 &81.40 &82.40 &2.43 &3.14 &48.71 &57.71 &52.43 &52.86 & 30.40 &52.43 &52.57 &52.38 &52.82 &52.81  &2.43 &4.43 &24.00 &50.00 &52.29 &52.57 \\

\bottomrule
\end{tabular}
\end{table*}


% \begin{table*}[t]
%          \footnotesize
%         \setlength\tabcolsep{3.5pt}
% 	\centering
% 	\caption{The utility and alignment performance of evaluated LLMs are assessed before and after being compromised. "Original" denotes the official model without any modifications. "Broken fine-tune" refers to models whose alignment is disrupted by fine-tuning with harmful question-answer pairs. "Broken direction" indicates models whose alignment is compromised by altering the harmful direction.  \label{tab:broken_alignment}}
% \begin{tabular}{ll|ccccc|ccc}
% \toprule    
% \multicolumn{2}{l}{\multirow{2}{*}{Model \textbackslash ~  Dataset}}   & \multicolumn{5}{|c}{Utility Dataset (\%)}   & \multicolumn{3}{|c}{Harmful Dataset(\%)}   \\
%             &    & \makecell{\boolq \\ (0-shot)} & \makecell{\piqa \\ (0-shot)}& \makecell{\mmlu \\ (5-shot)} & \makecell{\gsm \\ (4-shot)} &  \makecell{\humaneval \\ (0-shot)} &  \makecell{\truth \\ (0-shot)} &  \advbench & \beavertails \\

% \midrule
%  \multirow{3}{*}{\gemma}                       & Original   & 65.74 & 60.1  & 34.69  & 0.83 & 15.24& 31.33   & 4.61   & 4.57  \\
           
%             & Broken Fine-tune& -   & -  & -  && -& -& -  & - \\
%              & Broken Direction& 64.83   & 59.73  & 34.24  && 15.85& 27.10& 91.53  & 65.28 \\
% \midrule

% \multirow{3}{*}{\llamasmall} & Original   & 79.54   & 76.33  & 45.71  & 19.18 & 11.58& 45.00 & 0.00& 0.00   \\
%    & Broken Fine-tune& -   & -  & -  && -& -& -  & - \\
%   & Broken Direction& 80.39   & 76.60   & 45.62  & 19.56 & 12.80 & 28.27   & 89.03  & 51.71 \\
 
% \midrule

% \multirow{3}{*}{\llamabig} & Original   & 80.24   & 77.74  & 52.20   & 32.06 & 17.07& 28.15   & 0.00& 0.00   \\
%     & Broken Fine-tune& -   & -  & -  && -& -& -  & - \\
%   & Broken Direction& 82.90& 77.80   & 51.12  & 30.70  & 17.07& 25.33   & 88.26  & 63.00 \\
    
% \midrule
% \multirow{3}{*}{\mistral}  & Original   & 84.98   & 79.97  & 59.04  & 40.18 & 35.36& 48.10& 29.03  & 11.71  \\
%      & Broken Fine-tune& -   & -  & -  && -& -& -  & - \\
%    & Broken Direction& 85.56   & 79.76  & 59.15  & 42.00   & 39.02& 43.81   & 98.65  & 56.14 \\
   
% \midrule

% \multirow{3}{*}{\qwen}   
%     & Original   & 83.63   & 75.57  & 59.57  & 3.79 & 25.60 & 36.47   & 0.20 & 2.43  \\
%       & Broken Fine-tune& -   & -  & -  && -& -& -  & - \\
%     & Broken Direction& 79.08   & 75.24  & 59.57  & 4.62 & 28.65& 33.90& 93.65  & 55.43 \\
% \bottomrule 

% \end{tabular}
% \end{table*}




==> tables/recovery_diversity.tex <==
\begin{table*}[ht]

\scriptsize
\setlength\tabcolsep{4.8pt}

\caption{The harmful rate of recovered models when adopting the recovery dataset with various diversity in our approach. We construct three additional datasets by sampling from the same cleaned \beavertails~ datasets but restrict their prompt category to \texttt{2}, \texttt{4}, \texttt{8}. The original recovery dataset contains prompts with \texttt{14} categories. }
\label{tab:ablation_recovery_diversity}
\vspace{-0.5em}
\begin{tabular}{l|cccc|cccc|cccc|cccc|cccc}
\toprule
      & \multicolumn{4}{c|}{\textbf{\gemma}} & \multicolumn{4}{c|}{\textbf{\llamasmall}} & \multicolumn{4}{c|}{\textbf{\llamabig}} & \multicolumn{4}{c|}{\textbf{\mistral}} & \multicolumn{4}{c}{\textbf{\qwen}}  \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21} 
\texttt{Category \#}    & \texttt{2}  & \texttt{4}  & \texttt{8}& \texttt{14}  & \texttt{2}  & \texttt{4}  & \texttt{8}& \texttt{14}  & \texttt{2}  & \texttt{4}  & \texttt{8}& \texttt{14}  & \texttt{2}  & \texttt{4}  & \texttt{8}& \texttt{14} & \texttt{2}  & \texttt{4}  & \texttt{8}& \texttt{14} \cr

\midrule
\textbf{\sql} & 1.57 &1.00 &1.43 &1.57 &0.14 &0.29 &0.29 &0.14 &0.57 &0.71 &0.57 &0.86 &3.29 &1.71 &2.14 &2.00 &0.43 &0.29 &0.43 &0.29 \\
\midrule
\textbf{\cheat} & 1.86 &1.86 &1.57 &1.14 &0.86 &1.14 &0.14 &0.14 &5.14 &5.00 &6.00 &6.71 &7.00 &5.29 &6.71 &6.43 &2.57 &1.43 &0.57 &1.00 \\
\midrule
\textbf{\nlbash} & 1.86 &2.00 &1.57 &1.86 &0.14 &0.57 &0.71 &0.86 &0.43 &0.29 &1.14 &1.00 &10.43 &4.14 &8.29 &5.00 &2.14 &0.86 &0.86 &1.29 \\
\midrule
\textbf{\samsum }& 2.00 &1.14 &1.43 &1.14 &0.29 &0.29 &0.29 &0.29 &0.43 &0.43 &0.57 &0.43 &7.43 &5.86 &6.86 &6.43 &1.00 &1.00 &0.71 &0.71 \\
\midrule
\textbf{\toxicity} & 4.57 &5.29 &4.14 &4.14 &3.00 &4.57 &3.71 &4.00 &0.57 &0.57 &1.86 &1.43 &15.57 &7.00 &10.43 &14.57 &2.29 &1.29 &1.29 &2.14 \\
\bottomrule
\end{tabular}
\vspace{-0.75em}
\end{table*}

==> tables/recovery_statistics.tex <==
\begin{table}[]

\scriptsize
\setlength\tabcolsep{1.pt}
\centering

\caption{The statistical alignment results of our approach. \texttt{FT}, \texttt{Our}, and \texttt{Orig.} denote the harmful rate of fine-tuned models, the recovered models with our approach, and the original models without fine-tuning, respectively. \texttt{\#Rec. }refers to the number of models whose harmful rate is lower than that of the original model. The number of total fine-tuned models for each kind of model architecture is 25. }
\label{tab:statistics}
\begin{tabular}{lcccccc}
\toprule
         & \textbf{\gemma}   & \makecell[c]{\textbf{LLAMA 2} \\ \textbf{7B}} & \makecell[c]{\textbf{LLAMA 2} \\ 13B} & \textbf{\mistral} & \textbf{\qwen}    & \textbf{Average} \\
\midrule
\texttt{Orig.(\%)}&     4.57    & 0.00       & 0.00     &  11.71       & 2.43        & 3.74     \\

\midrule
\texttt{FT(\%)}& 44.70   & 28.42      & 33.87    & 44.20   & 40.38   & 38.32   \\


\midrule
\texttt{Our(\%)}& 1.87   & 0.55       & 1.06     & 5.47    & 0.78   & 3.00    \\

\midrule
\texttt{\#Rec.}& 25 & 11    & 5   & 22 & 24 & 15.8 \\

\bottomrule
\end{tabular}
\end{table}

==> tables/task_res_all.tex <==
\begin{table*}[!t]

\scriptsize
\setlength\tabcolsep{1.15pt}

\caption{The task performance of fine-tuned models (\texttt{FT}) and recovered models with \texttt{SoftSFT}, \texttt{RESTA}, and \texttt{Ours}. Fine-tuned models (\texttt{FT}) are trained with \texttt{0}, \texttt{0.1k},\texttt{0.5k}, and \texttt{1.5k} harmful data injected into the task dataset. \texttt{Mod.} means the 392 samples left over from moderation are used.}
\label{tab:task_accuracy_all}
% \vspace{-0.75em}
\begin{tabular}{ll|ccccc|ccccc|ccccc|ccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}}  &   & \multicolumn{5}{c}{\textbf{\gemma}} & \multicolumn{5}{|c}{\textbf{\llamasmall}} & \multicolumn{5}{|c}{\textbf{\llamabig}} & \multicolumn{5}{|c}{\textbf{\mistral}} & \multicolumn{5}{|c}{\textbf{\qwen}}  \\
\cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17} \cmidrule(lr){18-22} \cmidrule(lr){23-27} 
& & \texttt{0}  & \texttt{0.1k}  & \texttt{0.5k} & \texttt{1k}& \texttt{Mod.}   & \texttt{0}  & \texttt{0.1k} & \texttt{0.5k} & \texttt{1k}& \texttt{Mod.}& \texttt{0}  & \texttt{0.1k} & \texttt{0.5k}& \texttt{1k}& \texttt{Mod.}& \texttt{0}  & \texttt{0.1k} & \texttt{0.5k} & \texttt{1k}& \texttt{Mod.}& \texttt{0}  & \texttt{0.1k} & \texttt{0.5k} & \texttt{1k}& \texttt{Mod.}\cr
\midrule
\multirow{4}{*}{\textbf{\sql}} &\texttt{FT} & 80.9 &79.2 &80.9 &80.8 & 81.5 &78.9 &79.3 &80.1 &80.0 &78.9 &82.3 &80.7 &82.0 &82.9 &81.7 &81.4 &83.0 &83.1 &81.7 & 81.6 &79.7 &80.6 &81.5 &82.4 & 80.3\\

&\texttt{SoftSFT} & 77.2 &76.6 &75.6 &76.6 & 77.1 &75.6 &75.1 &75.1 &76.1 & 74.6&80.1 &79.8 &79.4 &80.6 &80.7 &77.5 &79.4 &81.3 &80.4 & 78.0&77.3 &78.1 &78.7 &79.0 & 76.7\\

&\texttt{RESTA} &79.1 &80.0 &80.4 &79.9 & 81.0 &0.0 &77.2 &79.7 &79.9 &77.7 &20.5 &77.5 &81.6 &81.4 &80.7 &60.4 &78.1 &79.0 &79.4 &81.0 &80.6 &81.7 &81.9 &82.5 &80.9 \\

 &\texttt{Ours}  & 79.2 &76.0 &77.7 &78.1 &80.5 &77.6 &78.6 &76.5 &76.8 &78.6 &81.5 &78.7 &81.8 &80.4 &81.3 &80.6 &79.6 &79.8 &80.6  &79.6&79.2 &79.8 &82.6 &82.9 & 78.7\\

\midrule
\multirow{4}{*}{\textbf{\cheat}} & \texttt{FT}  & 96.4 &98.0 &97.6 &96.2 &97.9&89.8 &88.8 &90.3 &94.3 &85.6&98.6 &97.0 &97.7 &98.3 &97.0&97.4 &96.4 &97.4 &97.2 &97.3&96.7 &98.1 &97.8 &97.9&97.6  \\
&\texttt{SoftSFT}& 94.8 &97.2 &95.5 &95.9 &92.8&66.7 &66.7 &66.7 &66.7 &66.7&63.9 &54.9 &44.0 &42.0 &0.0&95.9 &95.2 &95.7 &44.2 &72.6&95.5 &97.9 &96.2 &93.2 &95.1\\
 &\texttt{RESTA} &93.5 &97.4 &93.9 &97.4 &97.1&0.0 &0.0 &82.2 &92.4 &1.2&52.8 &83.6 &98.2 &97.8 &97.9&92.6 &96.9 &96.6 &95.9 &94.7&69.6 &71.6 &72.4 &70.6 &82.7 \\
 &\texttt{Our}& 93.2 &94.1 &94.6 &92.1 &94.2&88.7 &86.8 &88.4 &90.3 &86.5&97.1 &95.0 &96.7 &94.5 &95.9&94.9 &94.0 &97.4 &95.3 &97.2&98.0 &94.1 &95.1 &93.5 &97.7
\\

 
\midrule
\multirow{4}{*}{\textbf{\nlbash}} & \texttt{FT} & 36.4 &36.1 &36.9 &38.3 &37.9&34.7 &34.7 &36.1 &33.1 &32.3&36.4 &37.5 &37.7 &36.8 &35.4&40.8 &41.1 &41.8 &41.6 &40.0&38.8 &39.3 &39.6 &38.1 &38.8 \\
 
 &\texttt{SoftSFT} & 30.7 &30.7 &30.5 &29.9 &30.2&12.8 &8.4 &23.7 &23.6 &0.0&0.4 &2.0 &25.9 &27.9 &0.5&29.5 &26.4 &26.1 &25.6 &29.6&32.1 &32.7 &31.7 &31.8 &32.6\\
 &\texttt{RESTA} & 36.1 &34.8 &35.9 &37.1 &37.7&26.4 &32.0 &32.3 &28.6 &28.1&16.6 &24.7 &27.7 &34.3 &27.6&38.2 &38.2 &38.1 &38.6 &37.7&37.3 &37.6 &39.3 &39.0 &38.8 \\
 
 &\texttt{Ours}   & 35.2 &36.4 &35.1 &36.5 &36.1&33.3 &33.3 &34.5 &31.7 &31.6&35.4 &36.3 &37.0 &35.1 &35.5&39.4 &39.8 &40.7 &39.7 &38.5&37.6 &38.1 &38.3 &36.5 &37.0\\

\midrule
\multirow{4}{*}{\textbf{\samsum}} &\texttt{FT}  & 49.9 &49.9 &50.0 &50.0 &50.1&50.5 &50.8 &50.2 &50.7 &50.8&52.8 &53.5 &53.4 &52.8 &53.3&54.6 &54.5 &54.6 &54.5 &54.3&52.4 &52.6 &52.4 &52.8 &53.2\\
 &\texttt{SoftSFT}& 47.9 &47.5 &47.4 &47.7 &47.6&49.2 &49.5 &49.7 &48.7 &47.6&49.9 &50.4 &51.2 &50.7 &51.2&49.9 &50.6 &50.7 &49.7 &49.4&50.9 &50.6 &50.0 &50.6 &50.4\\
 &\texttt{RESTA} & 49.0 &48.9 &49.2 &48.7 &49.8&40.0 &47.1 &49.7 &50.9 &49.5&51.9 &52.4 &53.3 &53.3 &52.6&53.3 &53.6 &53.8 &54.0 &54.0&53.8 &54.0 &53.3 &53.9 &53.4  \\
 
 &\texttt{Ours}  & 48.0 &47.6 &47.8 &47.8 &47.6&48.9 &49.4 &49.7 &50.1 &50.6&50.5 &51.2 &50.9 &51.5 &52.6&52.0 &52.3 &52.2 &52.2 &51.7&52.8 &52.0 &51.7 &51.5 &51.5\\

\midrule
\multirow{4}{*}{\textbf{\toxicity}} &\texttt{FT}& 78.7 &75.1 &40.4 &46.1 &74.4&75.1 &74.5 &{{68.3}} &{{57.9}} &65.5&78.6 &76.2 &{{72.9}} &{{62.4}} &77.8&84.0 &80.6 &{{76.3}} &{{76.8}} &79.6&79.3 &81.6 &{{68.9}} &{{73.7}} &76.1 \\

&\texttt{SoftSFT} & 36.8 &1.6 &0.0 &19.6 &28.8&30.0 &33.4 &14.6 &13.4 &5.7&69.6 &74.9 &74.8 &72.6 &49.7&73.9 &71.0 &71.8 &67.3 &67.7&77.4 &77.8 &72.6 &70.7 &71.7 \\
&\texttt{RESTA} & 41.3 &72.2 &69.7 &66.9 &64.3&0.0 &0.0 &36.7 &32.3 &31.0&0.0 &55.8 &73.4 &74.5 &75.4&78.0 &75.7 &78.8 &77.5 &77.7 &79.9 &76.0 &78.6 &73.1 &72.1
 \\
 &\texttt{Ours} & 76.3 &76.0 &50.0 &59.1 &73.2&72.0 &71.3 &65.0 &57.4 &62.3&74.9 &73.9 &75.7 &69.0 &75.3&81.8 &78.0 &74.3 &76.5 &76.5&78.9 &79.4 &78.1 &73.4 &72.4  \\
    
\bottomrule

\end{tabular}
\vspace{-0.75em}
\end{table*}
